A Graph Grammar for Modelling RNA Folding

We propose a new approach for modelling the process of RNA folding as a graph transformation guided by the global value of free energy. Since the folding process evolves towards a configuration in which the free energy is minimal, the global behaviour resembles the one of a self-adaptive system. Each RNA configuration is a graph and the evolution of configurations is constrained by precise rules that can be described by a graph grammar.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{Alexander Heu{\ss}ner, Aleks Kissinger, Anton Wijs (Eds.):\\ 2nd Graphs as Models workshop (GaM 2016)\\
EPTCS 231, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.231.3}{10.4204/EPTCS.231.3}}
\pdfoutput=1

